MST-KD: Multiple Specialized Teachers Knowledge Distillation for Fair Face Recognition

As in school, one teacher to cover all subjects is insufficient to distill equally robust information to a student. Hence, each subject is taught by a highly specialised teacher. Following a similar philosophy, we propose a multiple specialized teacher framework to distill knowledge to a student network. In our approach, directed at face recognition use cases, we train four teachers on one specific ethnicity, leading to four highly specialized and biased teachers. Our strategy learns a project of these four teachers into a common space and distill that information to a student network. Our results highlighted increased performance and reduced bias for all our experiments. In addition, we further show that having biased/specialized teachers is crucial by showing that our approach achieves better results than when knowledge is distilled from four teachers trained on balanced datasets. Our approach represents a step forward to the understanding of the importance of ethnicity-specific features.

==> sections/trash.tex <==
\section{State of the Art} \label{sec:sota}

This chapter summarizes the current literature on bias mitigation (Section \ref{sec:bias_SOTA}) and knowledge distillation (Section \ref{sec:KD_SOTA}). In Section \ref{sec:KD_bias}, the previously presented concepts meet to explain how KD methodologies have been used so far to address bias mitigation.

\subsection{Bias Mitigation} \label{sec:bias_SOTA}
%% 2. SOTA - Datasets
To analyze the performance differences between demographic groups associated with bias, it is necessary to provide a suitable test framework that allows a comparison based on the different sub-populations. Wang~\textit{et al.}~\cite{wang2019racial} proposed the Racial Faces in the Wild (RFW) dataset, which contains an equal percentage of impostor-genuine pairs from Caucasian, Indian, Asian and African identities. Similarly, Karkkainen~\textit{et al.}~\cite{karkkainen2021fairface} proposed FairFace, a race-balanced dataset that is diverse in terms of race, age, expressions, head orientation, and photographic conditions. Robinson~\textit{et al.}~\cite{robinson2020face} proposed another balanced dataset in terms of race, gender and both gender and race, Balanced Faces in the Wild (BFW). Wang~\textit{et al.}~\cite{wang2021meta} developed two novel datasets that follow distinct skin-tone distributions: real-world distribution (BUPT-Globalface) and equal proportions among the four considered ethnicities (BUPT-Balancedface).

Besides data-based bias mitigation strategies, model-based approaches have been proposed to increase the fairness of biometric models. Wang~\textit{et al.}~\cite{wang2021meta} evaluated the performance differences from the different complexity levels of the analyzed demographic sub-groups. The authors considered different adaptive margins for the evaluated skin tones, resulting in a better alignment of the model's feature space with the real data distribution, as harder skin tones can be assigned larger margins. Xu~\textit{et al.}~\cite{xu2020investigating} aimed to mitigate bias in facial emotion recognition by either removing the sub-group attribute information or highlighting it during their recognition process. Franco~\textit{et al.}~\cite{franco2021learn} increased fairness by making the models learn fair representations of the input samples, considering that the distributions of the representation vectors are independent of the attribute that can induce bias.

\section{Knowledge Distillation} \label{sec:KD_SOTA}
\subsection{Knowledge Distillation for Model Compression}
KD algorithms have already been used to aid the development of lighter models in the biometrics area, namely in FR. Boutros~\textit{et al.}~\cite{boutros2022pocketnet} used a multistep KD (MS-KD) methodology to distill knowledge to a lightweight student network used in FR applications with limited memory specifications, resulting in increased performance. Wang~\textit{et al.}~\cite{wang2021teacher} studied FB-KD using a validation loss with a term that estimates the computational cost of the defined model, $L_{comp}$. This allows for the utilization of Neural Architecture Search (NAS) \cite{zoph2016neural} to optimize the student's architecture. Luo~\textit{et al.}~\cite{luo2016face} considered a loss term that does not comprise all the neurons of each layer since the neurons in the middle of the network encode information regarding different characteristics of the analyzed faces. This information includes attributes relevant to the FR task such as race and gender, and non-related attributes that should not influence the algorithm \cite{luo2016face}. Hence, this strategy allows for penalizing irrelevant or redundant neurons, reducing their impact on the KD process.

However, KD algorithms are not restricted to model compression and acceleration tasks. Huber~\textit{et al.}~\cite{huber2021mask} bridged the accuracy gap of FR models in masked faces by distilling knowledge from a teacher trained on unmasked faces to a student trained on both masked and unmasked faces with remarkable results. KD was also used to bridge the performance gap between models trained on high and low-resolution images. Ge~\textit{et al.}~\cite{ge2018low} used FB-KD to distill knowledge from a teacher trained on high-resolution images to a student trained on their low-resolution versions. This strategy penalized the distillation contribution given by outliers to avoid transferring information that negatively impacts the student's performance. Caldeira~\textit{et al.}~\cite{caldeira2023unveiling} focused on the binary task of morphing attack detection, distilling distinct types of knowledge depending on each sample's class, achieving competitive results.

Although distilling knowledge from a single teacher can highly benefit the student's performance, it might lead to undesired situations such as the distillation of biased predictions that can be at least partially alleviated when knowledge is distilled from several sources \cite{caldeira2024model}. The first multi-teacher KD methods proposed simple strategies to integrate the teachers' knowledge before distilling it to the student, namely attributing fixed weights to each teacher \cite{you2017learning, fukuda2017efficient, wu2019multi} to give them different importance levels in the distillation. These methods were soon classified as suboptimal since the relative importance of each teacher should be determined with finer granularity, as the teachers' relative capacity varies depending on the considered sample \cite{zhang2022confidence} and the layer from where knowledge is being distilled \cite{pham2023collaborative}, which cannot be trivially predicted. Xu~\textit{et al.}~\cite{xu2023probabilistic} used KD to generate a student model from an ensemble of teachers, weighing each teacher's importance in a sample-wise manner. Pham~\textit{et al.}~\cite{pham2023collaborative} presented an online distillation method for quantized networks, where the teachers and student networks are trained simultaneously, allowing the weight attributed to each teacher to be learned during the training process, which facilitates their optimization. Zhang~\textit{et al.}~\cite{zhang2022confidence} combined the teachers' knowledge with different weights for each training sample, depending on the teachers' relative level of confidence in their classification, measured as the cross-entropy between its predictions and the ground truth labels.    

% A recurrent problem in knowledge distillation is the existence of a capacity gap between teacher and student that can result in low compatibility between their spaces. While in compression this gap can be attributed to the different complexity of teacher and student networks \cite{luo2016face,li2023rethinking}, when KD is adopted to mitigate data issues, this gap is associated with the different amounts of information these models have access to \cite{aslam2023privileged}. The concept of multiple teachers can be used to close this gap \cite{zhang2023adaptive, xu2022knowledge}. Zhang~\textit{et al.}~\cite{zhang2023adaptive} focused on integrating compatible knowledge between the teachers' ensemble and the student through a meta-learning process where the student is trained at the same time as a network that aggregates the teachers’ knowledge with the current student's state. These networks are responsible for extracting the weights that will be used to weigh each teacher's influence in the RB-KD and FB-KD of the final loss terms. The authors verify that multi-teacher KD methods generally surpass single-teacher KD and that the proposed methodology surpasses previous multi-teacher KD strategies. Xu ~\textit{et al.}~\cite{xu2022knowledge} suggests that transferring knowledge from an ensemble where all the teachers have the same architecture as the student can lead to good results, while completely removing the complexity gap between each teacher and the student network. The authors show that using a single complex teacher results in a higher average probability for the predicted class, while an ensemble of homogeneous teachers leads to a softer probability distribution. This idea follows a similar line of thought as using RB-KD instead of the hard ground truth labels: softening the labels can give more information because it reveals some inter-class relations that would be otherwise omitted, revealing the potential of performing KD from a set of homogeneous teachers. The proposed multi-teacher KD method resulted in a performance boost when compared with traditional KD and proved to be efficient in comparison with transferring knowledge from a heterogeneous ensemble.

% Kong~\textit{et al.}~\cite{kong2024dual} developed a dual-teacher KD approach to train a student on the face anti-spoofing task. Due to the low data availability for this task, the knowledge is transferred from teachers trained in FR and face attribute editing (FAE), since the priors produced by these models contain knowledge on facial features that can be useful to the student. This model is composed of a backbone followed by three parallel prediction headers that share the same feature space. The headers trained on FR and FAE receive knowledge from the teacher models while the face anti-spoofing header uses the cross-entropy loss. When compared with a baseline model trained only with the face anti-spoofing branch, models trained with a single teacher generally achieve better performances and lower error rates. Simultaneously, using both teachers to perform the knowledge distillation leads to better results than using either of them individually, proving the usefulness of multi-teacher KD.

% Shao~\textit{et al.}~\cite{shao2023multi} used a multi-teacher KD approach to improve cross-dataset palmprint recognition. In this type of scenario, there is a source dataset and several target datasets to which the model should be deployed; the differences between these datasets can be the illumination level of the images, for example. Training a model directly on all these datasets generally leads to reduced performance because it is hard to create a space that is simultaneously appropriate to all of them. In this multi-teacher approach, the source dataset is used to train all the teachers in a supervised manner. Simultaneously, each teacher processes images of one of the target datasets; these images are not used in the supervised training, but they should produce similar features and convolution maps to the source dataset samples of the same identity. This similarity can be incorporated into the teacher’s training function through an extra loss term that adapts the teacher's capacity to work for both the source and that specific target dataset. Then, the teachers transfer knowledge to a final student trained on all the datasets. This approach surpassed a student model trained with the ArcFace loss \cite{deng2018arcface} alone on all the datasets and resulted in a significant improvement when compared with SOTA methodologies on palmprint recognition.

% Although the work developed by Shao~\textit{el al.}~\cite{shao2023multi} focuses on palmprint recognition and does not relate to racial bias mitigation, their strategy presents some resemblances with the methodology proposed in this document. In our problem, we split a dataset with face images into specific demographic groups according to the ethnicity of each identity. Although all subsets originate from the same dataset, the clear distinction between them resembles what happens in cross-dataset problems. Furthermore, the concept of source dataset is not relevant to our work, but each of the teacher models used in the KD procedure is fed information from a different subset and is then used to distill knowledge to a student trained on all images, similarly to what happens in Shao~\textit{el al.}~\cite{shao2023multi}. It should also be noted that the best-performing methodology proposed in this work, AF-Fusion, uses a set of learned weights. Despite distilling from 4 teachers, our approach learns $2048\times512$ weights, as the feature vector inputted to the adaptor is constructed from a linear combination of all features returned by the four teachers. The following section further shows the use of KD for a similar purpose to ours: demographic bias mitigation.

\section{Knowledge Distillation for Bias Mitigation} \label{sec:KD_bias}
Liu~\textit{et al.}~\cite{DBLP:conf/iccvw/LiuZSYL21} proposed two strategies to extract a more uniform subsample of the considered training set, to ensure that useful knowledge is distilled during the KD procedure. These strategies outperformed simple KD in the evaluated scenarios, resulting in a significant improvement in fairness. As compressing a model can easily lead to increased bias levels \cite{caldeira2024model}, Blakeney~\textit{et al.}~\cite{blakeney2021simon} used KD to fine-tune a pruned network, proving that KD effectively reduced the pruning-induced bias, resulting in fairer models.

As previously stated, the present work also proposes a framework that uses KD to mitigate racial bias. This is done through the separation of a balanced dataset into four subsets divided by ethnicity. A teacher model is then assigned to each of these subsets and trained on it, resulting in four teachers whose extracted features are used to perform KD to a student trained on samples from all ethnicity groups. 
